Evaluating Adversarial Robustness in the Spatial Frequency Domain

Convolutional Neural Networks (CNNs) have dominated the majority of computer vision tasks. However, CNNs' vulnerability to adversarial attacks has raised concerns about deploying these models to safety-critical applications. In contrast, the Human Visual System (HVS), which utilizes spatial frequency channels to process visual signals, is immune to adversarial attacks. As such, this paper presents an empirical study exploring the vulnerability of CNN models in the frequency domain. Specifically, we utilize the discrete cosine transform (DCT) to construct the Spatial-Frequency (SF) layer to produce a block-wise frequency spectrum of an input image and formulate Spatial Frequency CNNs (SF-CNNs) by replacing the initial feature extraction layers of widely-used CNN backbones with the SF layer. Through extensive experiments, we observe that SF-CNN models are more robust than their CNN counterparts under both white-box and black-box attacks. To further explain the robustness of SF-CNNs, we compare the SF layer with a trainable convolutional layer with identical kernel sizes using two mixing strategies to show that the lower frequency components contribute the most to the adversarial robustness of SF-CNNs. We believe our observations can guide the future design of robust CNN models.

==> apx/B_additional_experiments/gradcam_simple.tex <==
\captionsetup[subfigure]{labelformat=empty}
\begin{figure*}[t]
    \centering
    % Golf
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/golf.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgolf_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgolf_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/golf_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbgolf_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgolf_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/golf_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgolf_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgolf_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/golf_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgolf_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgolf_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    % gas
    \centering
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/gas.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgas_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgas_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/gas_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgas_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgas_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/gas_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgas_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgas_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/gas_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgas_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgas_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    % parachute
    \centering
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/chute.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchute_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchute_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/chute_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchute_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchute_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/chute_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchute_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchute_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/chute_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchute_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchute_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    % chain saw
    \centering
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/saw.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbsaw_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fsaw_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/saw_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbsaw_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fsaw_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/saw_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbsaw_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fsaw_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/saw_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbsaw_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fsaw_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    % church
    \centering
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/church.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchurch_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchurch_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/church_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchurch_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchurch_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/church_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchurch_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchurch_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/church_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchurch_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchurch_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    \caption{Grad-Cam visualization of VGG11 based transfer attacks. Top, middle and bottom of each column presents the (adversarial) image, visualization of ResNet18 and that of SF-ResNet18.}
    \label{apxfig:grad_cam}
\end{figure*}   

\begin{figure*}[t]
    \centering
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/golf.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgolf_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgolf_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/golf_f01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbgolf_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fgolf_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/golf_f02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbgolf_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fgolf_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/golf_f03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbgolf_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fgolf_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    %gas pump
    \centering
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/gas.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbgas_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fgas_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/gas_f01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbgas_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fgas_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/gas_f02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbgas_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fgas_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/gas_f03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbgas_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fgas_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    % parachute
    \centering
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/chute.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_rgbchute_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/cam_fchute_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/chute_f01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbchute_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fchute_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/chute_f02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbchute_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fchute_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}{.075\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/apx/chute_f03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_rgbchute_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/apx/fcam_fchute_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    \caption{Grad-Cam visualization of SF-VGG11 based transfer attacks. Top, middle and bottom of each column presents the (adversarial) image, visualization of ResNet18 and that of SF-ResNet18.}
    \label{apxfig:grad_cam_sf}
\end{figure*}   


==> apx/bin/0_main.tex <==


    % The input images are first linearly transformed from the RGB color space to the YCbCr color space, where $Y$ represents the overall brightness, while $Cb$ and $Cr$ denote the chrominance in blue and red~\cite{yang2007fast}, as follows.
    % \begin{equation}\small
    %     \begin{bmatrix}
    %     Y \\ Cb \\ Cr
    %     \end{bmatrix} 
    %     =
    %     \begin{bmatrix}
    %     0.257 & 0.504 & 0.098 \\ 
    %     0.439 & -0.368 & -0.071 \\ 
    %     -0.148 & -0.291 & 0.439 
    %     \end{bmatrix}
    %     \begin{bmatrix}
    %     R \\ G \\ B 
    %     \end{bmatrix}
    %     + 
    %     \begin{bmatrix}
    %     16 \\ 128 \\ 128
    %     \end{bmatrix}.
    % \end{equation}
    % Note that here the $R, G, B$ are integer values in the range $[0, 255]$. Next, after translating to the YCbCr space, 
    
    
    % Notice that our investigation of spatial frequency is inspired by relevant biological research on the human visual systems (HVS)~\cite{bruce2003visual, tovee1996introduction}. In particular, while Hubel and Wiesel hypothesize that visual neurons react to straight edges and lines~\cite{hubel1965receptive}, subsequent biological evidences suggest that human visual systems utilize spatial frequency channels~\cite{shapley1985spatial}. In particular, it is hypothesized that HVS utilizes spatial frequency channels~\cite{hall1977nonlinearspatial} and filters spatial data using arrays of cells selective for spatial frequency~\cite{field1993contour}. However, as CNN is inspired by Hubel's and Wiesel's finding~\cite{lecun1998gradient}, it did not incorporate the latter findings regarding spatial frequency components. Thus, we are intrigued to investigate whether the robustness of CNN may improve by incorporating the frequency domain.



% \noindent\textbf{Remark.}
% \subsubsection{Spatial frequency in human visual systems}
% tootell1988functional, slaghuis1999spatial, issa2000spatial

% the compared works: https://www.one-tab.com/page/bcL_apNrSVGw3DsmvxFZ0Q

==> apx/bin/2_C88_SPF.tex <==
\subsection{The SF layer formulated as a $C_{88}$ layer}
\label{apx:SPF_as_C88}
    The DCT formula is repeated below for clarity. With a $8\times8$ matrix $\mathbf{B}$ denoting one of the three colors of an $8\times8$ pixel patch, we obtain the spacial frequency matrix $\mathbf{D}$ as
    \begin{align}\small
        \label{apxeqn:DCT}
        \mathbf{D}_{u,v}&= \sum _{x=0}^7\sum _{y=0}^7\mathbf{B}_{x,y}\mathbf{K}_{x,y}^{u,v}\\
        \label{apxeqn:DCT_kernel}
        \mathbf{K}_{x,y}^{u,v} &= 
        \frac{c(u)c(v)}{4}\cos \left[{\frac {(2x+1)u\pi }{16}}\right]
        &\cos \left[{\frac {(2y+1)v\pi }{16}}\right]
    \end{align}
    with the normalizing coefficient $c$ defined as
    \begin{equation}
        c(u)=\begin{cases}\frac{1}{\sqrt{2}}, & \text{if } u = 0\\ 1, & \text{otherwise} \end{cases}
    \end{equation}
    
    
    

==> apx/bin/3_basis_zigzag.tex <==



==> apx/bin/4_frequency_attack.tex <==
\subsection{Perturbation on the frequency domain}
\label{subsec:4-4FrequencyAttack}

\begin{table*}[ht]\small
    \centering
    \begin{tabular}{lc|cc c|cc c|cc}
    \toprule
    &\multicolumn{3}{c}{ImageNette} & \multicolumn{3}{c}{CIFAR10} & \multicolumn{3}{c}{Flower102}\\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    model 
    & Acc. &  $\epsilon=0.003$ & $\epsilon=0.01$ 
    & Acc. &  $\epsilon=0.003$ & $\epsilon=0.01$ 
    & Acc.&  $\epsilon=0.003$ & $\epsilon=0.01$ \\
    \midrule
    SF-ResNet18 & $80.8\%$ & $5.6\%$ & $0.0\%$ & $78.0\%$ & $17.5\%$ & $0.1\%$ & $75.1\%$ & $21.5\%$ & $0.0\%$\\
    ResNet18 & $80.2\%$ & $0.0\%$ & $0.0\%$ & $78.0\%$ & $0.0\%$ & $0.0\%$ & $74.0\%$ & $0.0\%$ & $0.0\%$\\
    (improvement) && ($+5.6\%$) & (+$0.0\%$)  && ($+17.5\%$) & ($+0.1\%$)  && ($+21.5\%$) & ($+0.0\%$) \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    SF-EfficientNet & $74.0\%$ & $8.8\%$ & $0.2\%$ & $77.0\%$ & $1.5\%$ & $0.0\%$ & $80.1\%$ & $29.2\%$ & $0.1\%$\\
    EfficientNet & $74.0\%$ & $0.0\%$ & $0.0\%$ & $79.8\%$ & $0.0\%$ & $0.0\%$ & $81.2\%$ & $0.1\%$ & $0.0\%$\\
    (improve) && ($+8.8\%$) & ($+0.2\%$)  && ($+1.5\%$) & ($+0.0\%$)  && ($+29.1\%$) & ($+0.1\%$) \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    SF-DenseNet & $78.2\%$ & $5.4\%$ & $0.2\%$ & $77.1\%$ & $0.0\%$ & $0.0\%$ & $73.0\%$ & $49.5\%$ & $5.6\%$\\
    DenseNet & $78.2\%$ & $0.6\%$ & $0.0\%$ & $79.2\%$ & $0.0\%$ & $0.0\%$ & $71.4\%$ & $0.0\%$ & $0.0\%$\\
    (improvement) && ($+5.4\%$) & ($+0.2\%$)  && ($+0.0\%$) & ($+0.0\%$)  && ($+49.5\%$) & ($+5.6\%$) \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    SF-VGG11 & $78.8\%$ & $1.0\%$ & $0.0\%$ & $78.6\%$ & $11.5\%$ & $0.0\%$ & $70.1\%$ & $6.5\%$ & $3.4\%$\\
    VGG11 & $78.6\%$ & $0.0\%$ & $0.0\%$ & $79.0\%$ & $0.0\%$ & $0.0\%$ & $70.9\%$ & $0.0\%$ & $0.0\%$\\
    (improvement) && ($+1.0\%$) & ($+0.0\%$)  && ($+11.5\%$) & ($+0.0\%$)  && ($+6.5\%$) & ($+3.4\%$) \\
    \bottomrule 
    \end{tabular}
    \caption{Test accuracy of the images under attack on frequency domain (larger is better). The ``Acc.'' columns denotes the test accuracy without adversarial attack. The (improvement) rows denotes the percentage of improvements of attacked accuracy for SF-CNN models over the CNN models.}
    \label{tab:exp_1_norm_bound_asr_freq}
\end{table*}


==> apx/bin/a_visualization/index.tex <==
\section{Grad-Cam on adversarial images}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/test1.eps}
        \includegraphics[width=.98\linewidth]{figure/cam_RGB.eps}
        \includegraphics[width=.98\linewidth]{figure/cam_f.eps}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/VGGadv_01_1.eps}
        \includegraphics[width=.98\linewidth]{figure/cam_RGB_01.eps}
        \includegraphics[width=.98\linewidth]{figure/cam01_f.eps}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/VGGadv_02_1.eps}
        \includegraphics[width=.98\linewidth]{figure/cam_RGB_02.eps}
        \includegraphics[width=.98\linewidth]{figure/cam02_f.eps}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/VGGadv_03_1.eps}
        \includegraphics[width=.98\linewidth]{figure/cam_RGB_03.eps}
        \includegraphics[width=.98\linewidth]{figure/cam03_f.eps}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    \caption{Grad-Cam on adversarial images generated by VGG. Upper row is the adversarial images of different size of $\epsilon$. Medium row is results of Grad-Cam for ResNet18 and below is for $f\dash$ResNet18. These figures show that ResNet18 would diverse the red area and can not focus on the main object of the image after increasing the $\epsilon$ norm.}
    \label{apxfig:grad_cam}
\end{figure}

==> apx/bin/b_detection/index.tex <==
 % Based on the above observation, we present the following detection method for the imagenette dataset, which can easily be extended to other datasets. Since the DCT coefficients of high frequency for Y, Cb and Cr color space shows similar patterns, we arbitrarily select the high frequency DCT coefficients of the Cr color space for the detection of adversarial examples, \jy{which we flatten to a  dimension of $1\times...$}.
    % flatten to a ? element vector 
    % \jy{if use distribution, describe process.} 
    
    % [red]
    % random
    % equal space
    
    % We design the $f\dash$Detector model, a basic $5\dash$layer DNN model with \jy{?} input neurons, 4096 hidden neurons and ReLU activation for each of the $3$ hidden layer and a single output neuron in the output layer. The $f\dash$Detector is trained with the the commonly-used binary? categorical cross entropy loss [cite] over normal and adversarial values using the SGD optimizer [cite] with a learning rate of $0.01$. 
    
    
    % \kh{DCT process spilt image to images blocks and each contain 192 channels DCT coefficients which is sorted from low frequency to high frequency. Therefore, we firstly selected the last 48 channels as high frequency components. Since DCT process has already transferred images into YCbCr color space, the order of channels would be in ${Y_1,Cb_1,Cr_1,Y_n,Cb_n,Cr_n}$ sequence. At last, we choose Cr information for each blocks and flatten it to a one dimension vector.}
    
    % \kh{For comparison, we apply a similar procedure to design the $p$-Detector, which represent a detector model trained on RGB pixel values. We report that a basic DNN fails to detect RGB pixel distribution successfully. To take a step further, we follow \cite{metzen2017detecting} to utilize ResNet18 as a backbone feature extraction, and attempt to detect on the resulting features. 
    
    % feature dimension?
    % DNN layer information?
    
    % After training with similar training procedure as above, we obtain the result in below.}
    
    % \kh{As shown in \cref{tab:exp_detector}, $f\dash$Detector achieves almost perfect result in detecting both regular adversarial examples and frequency attack examples. In contrast, CNN$\dash$Detector gets the acceptable performance in regular adversarial examples, but fails in frequency attack examples.}
    
    
    
    
    % To better understand the utility of the proposed detection method in the frequency domain, we apply a similar procedure to RGB pixel values. Concretely, we train a basic CNN detector which extracts pixel values for detection. 
    % Both models are trained with $\epsilon=0.01$ adversarial examples and normal images. Moreover, we retain the same environment settings and do not make any image pre-processing.

==> apx/bin/b_table/white_box_table.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabular}{lc|cc c|cc c|cc}
    \toprule
    &\multicolumn{3}{c}{ImageNette} & \multicolumn{3}{c}{CIFAR10} & \multicolumn{3}{c}{Flower102}\\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    model & acc &  $\epsilon=0.003$ &
     $\epsilon=0.01$ & acc &  $\epsilon=0.003$ &
     $\epsilon=0.01$ & acc &  $\epsilon=0.003$ &
     $\epsilon=0.01$ \\
    \midrule
    $f\dash$ResNet18 & $80.8\%$ & $16.8\%$ & $61.2\%$ & $78\%$ & $19.5\%$ & $66\%$ & $75.1\%$ & $17.9\%$ & $60.5\%$\\
    ResNet18 & $77\%$ & $28.1\%$ & $82.1\%$ & $78\%$ & $21.8\%$ & $69\%$ & $74.0\%$ & $20.6\%$ & $77.9\%$\\
    (reduce) && $11.3\%$ & $20.9\%$  && $2.3\%$ & $3\%$  && $2.7\%$ & $17.4\%$ \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    $f\dash$EfficientNet & $74.1\%$ & $21.6\%$ & $70.8\%$ & $77\%$ & $31.2\%$ & $88.8\%$ & $80.1\%$ & $31.1\%$ & $87.5\%$\\
    EfficientNet & $74.1\%$ & $38.8\%$ & $96.2\%$ & $79.8\%$ & $66.5\%$ & $99.9\%$ & $81.1\%$ & $46\%$ & $95.9\%$\\
    (reduce) && $17.2\%$ & $25.4\%$  && $35.3\%$ & $11.1\%$  && $14.9\%$ & $8.4\%$ \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
    $f\dash$DenseNet & $78.2\%$ & $21.9\%$ & $63.8\%$ & $77.1\%$ & $24.3\%$ & $76\%$ & $73\%$ & $16.7\%$ & $55.4\%$\\
    DenseNet & $78.2\%$ & $23.2\%$ & $67.3\%$ & $79.3\%$ & $75.2\%$ & $99.1\%$ & $71.3\%$ & $24.7\%$ & $79.3\%$\\
    (reduce) && $0.9\%$ & $3.5\%$  && $50.9\%$ & $23.1\%$  && $8.0\%$ & $23.9\%$ \\
    \bottomrule 
    \end{tabular}
    \caption{Attack Success Rate (ASR) of norm-bounded attack evaluations (smaller is better). The acc columns denotes the test accuracy without adversarial attack. The (reduce) rows denotes the percentage of reduction of ASR for $f$CNN models over original models.}
    \label{tab:exp_1_norm_bound_asr}
\end{table*}

 % CIFAR-10 -> EfficientNetV2
 % Flower102 -> DenseNet

==> apx/bin/b_visualization/grad_cam.tex <==
\section{Grad-Cam on adversarial images}

\begin{figure}[h]
    \centering
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/sec4/horn.jpg}
        \includegraphics[width=.98\linewidth]{figure/sec4/cam_rgbhorn_00.jpg}
        \includegraphics[width=.98\linewidth]{figure/sec4/cam_fhorn_00.jpg}
        \caption{$\epsilon = 0$}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/sec4/horn_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/sec4/cam_rgbhorn_01.jpg}
        \includegraphics[width=.98\linewidth]{figure/sec4/cam_fhorn_01.jpg}
        \caption{$\epsilon = 0.1$}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/sec4/horn_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/sec4/cam_rgbhorn_02.jpg}
        \includegraphics[width=.98\linewidth]{figure/sec4/cam_fhorn_02.jpg}
        \caption{$\epsilon = 0.2$}
    \end{subfigure}
    \begin{subfigure}[t]{.24\linewidth}
        \centering
        \includegraphics[width=.98\linewidth]{figure/sec4/horn_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/sec4/cam_rgbhorn_03.jpg}
        \includegraphics[width=.98\linewidth]{figure/sec4/cam_fhorn_03.jpg}
        \caption{$\epsilon = 0.3$}
    \end{subfigure}
    \caption{Grad-Cam on adversarial images generated by VGG. Upper row is the adversarial images of different size of $\epsilon$. Medium row is results of Grad-Cam for ResNet18 and below is for $f\dash$ResNet18. These figures show that ResNet18 would diverse the red area and can not focus on the main object of the image after increasing the $\epsilon$ norm.}
    \label{apxfig:grad_cam2}
\end{figure}



==> sec/4_experiment/3_advtrain.tex <==
\subsection{Evaluation on adversarial training}
\label{subsec:4-3advtrain}

We compare SF-CNN and CNN models under adversarial training~\cite{madry2018towards}. Here we follow \cite{shafahi2019adversarial} to perform \emph{free adversarial training} over $\epsilon=0.03$ adversarial examples. The same adversarial training procedure is applied to both SF-ResNet18 and ResNet18.  
% and each minibatch of examples are retrained $20$ times. In addition, we combine adversarial training with frequency learning. The regular images and adversarial examples would undergo the DCT process and train with the same settings as SF-ResNet18 above.

As shown in \Cref{tab:adv_train}, even under adversarial training, SF-ResNet18 is more robust than ResNet18. In particular,  SF-ResNet18 obtains $0.2\%, 2.6\%$, and $7.9\%$ lower ASR than ResNet18 under $\epsilon=0.003$, $\epsilon=0.01$ and $\epsilon=0.03$, respectively, while maintaining the same test accuracy. The result validates the efficacy of utilizing the frequency domain in conjunction with adversarial defense methods.


\begin{table}[h]
    \centering
    \begin{tabular}{llccc}
    \toprule
    model & acc & $\epsilon=0.003$ & $\epsilon=0.01$ & $\epsilon=0.03$\\
    \midrule
    SF-ResNet18 & $76.2\%$ & $72.2\%$ & $65.4\%$ & $38.0\%$ \\
    ResNet18  &$76.2\%$ & $72.2\%$ & $63.4\%$ & $32.0\%$ \\
    \bottomrule 
    \end{tabular}
    \caption{Adversarially trained SF-ResNet18 and ResNet18 on the imagenette dataset. SF-ResNet18 models are more robust.}
    \label{tab:adv_train}
\end{table}
